Proving Regulatory Compliance: Full Compliance Against an Expressive Unconditional Obligation is coNP-Complete

Organisations are required to show that their procedures and processes satisfy the relevant regulatory requirements. The computational complexity of proving regulatory compliance is known to be generally hard. However, for some of its simpler variants the computational complexity is still unknown. We focus on the eight variants of the problem that can be identified by the following binary properties: whether the requirements consists of one or multiple obligations, whether the obligations are conditional or always in force, and whether only propositional literals or formulae can be used to describe the obligations. This paper in particular shows that proving full compliance of a model against a single unconditional obligation whose elements can be described using formulae is coNP-complete. Finally we show how this result allows to fully map the computational complexity of these variants for proving full and non compliance, while for partial compliance the complexity result of one of the variants is still missing.

==> sections/p1l-.tex <==
\section{Partial Compliance: 1L- is in P}\label{sec:1l-}

We show that the variant \textbf{1L-} is in \textbf{P} by proposing a solution based on the \emph{pattern approach}~\cite{patternscompliance} that proves partial compliance of this variant in polynomial time.

\subsection{A Brief Introduction to the Pattern Approach}\label{sec:patterns_intro}

The pattern approach checks whether a variant \textbf{nL-} is fully compliant. The verification is done independently for each obligation through a set of patterns that are generated from the obligation being verified. Depending on the obligation's type and its components a different set of patterns are generated. These patterns are referred to as $\Delta$-constraints (Definition~\ref{def:delta_param1}).

\begin{definition}[Parametrised $\Delta$-constraints]\label{def:delta_param1}

$\Delta$-constraints are evaluated over process blocks in a WF-net. Given an obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, depending on its type and parameters different sets of patterns are generated and their evaluation represents the following:

\begin{description}
\item[achievement] The function $\overline{A}\Delta(\neg \oblr, \oblt, \obld)$ generates the set of $\Delta$-constraints. This patterns are evaluated over the process blocks of the WF-net, and when a block satisfies one of the generated patterns it corresponds to: there exists a trace in the block where $\neg \oblr$ holds when a transition having $\oblt$ annotated is executed, and $\neg \oblr$ holds until a transition having $\obld$ annotated is executed. This means that the block contains a trace violating the given achievement obligation.

\item[maintenance] The function $\overline{M}\Delta(\neg \oblr, \oblt, \obld)$ generates the set of $\Delta$-constraints. This patterns are evaluated over the process blocks of the WF-Net, and when a block satisfies one of the generated patterns it corresponds to: there exists a trace in the block where $\neg \oblr$ holds when a transition having $\oblt$ annotated is executed, or for a trace where $\neg \oblr$ holds before a transition having $\obld$ annotated is executed. This means that the block contains a trace violating the maintenance obligation.
\end{description}
\end{definition}

The evaluation of a $\Delta$-constraint over a process block is computed by aggregating the evaluation of its sub-blocks, meaning that the evaluation of one of this constraints can be done over the representation of the WF-Net as a tree structure and is polynomial in terms of the nodes in the tree. The overall evaluation procedure is outlines as follows:

\begin{enumerate}
\item For each $\Delta$-constraint obtained from an obligation being evaluated:
\begin{enumerate}
\item For each transition having the trigger of the obligation in its annotation (\emph{trigger transition}), evaluate whether the pattern represented by the $\Delta$-constraint can be satisfied when considering this particular transition as the one starting an in force instance of the local obligation.
\begin{enumerate}
\item Classify each transition in the WF-Net.
\item Recursively classify a process block in the model by aggregating the evaluations of its sub-blocks.
\item If one or more process blocks satisfy the pattern, then there exist a trace in the WF-Net violating the local obligation in this particular in force instance started by the \emph{trigger transition} being currently considered.
\end{enumerate}
\end{enumerate}
\item If a violating trace is identified by the approach, then the WF-Net can be classified as \emph{not fully compliant} with the given local obligation. Otherwise, if no such trace is found, then the WF-Net is \emph{fully compliant}.
\end{enumerate}

\subsection{Adapting the Pattern Approach to Check Partial Compliance of \textbf{1L-}}

To use the \emph{patterns approach} to check for partial compliance of \textbf{1L-} we use an alternative parametrisation of the $\Delta$-constraints introduced in Definition~\ref{def:delta_param1}. We describe the alternative parametrisations and their behaviours in Definition~\ref{def:delta_adapt_a} and Definition~\ref{def:delta_adapt_m}.

\begin{definition}[Achievement Parametrisation for Partial Compliance]\label{def:delta_adapt_a}
An achievement obligation $\Obl^{a}\langle \oblr, \oblt, \obld\rangle$ can be parametrised into $\overline{M}\Delta(\oblr, \oblt, \obld)$ to generate $\Delta$-constraints. With this parametrisation, the patterns would be satisfied by the existence of a trace where $\oblr$ holds when a transition having $\oblt$ annotated is executed, or a trace where $\oblr$ holds before a transition having $\obld$ annotated is executed.  Such a trace, if it exists, satisfies the given local achievement obligation.
\end{definition}

\begin{definition}[Maintenance Parametrisation for Partial Compliance]\label{def:delta_adapt_m}
A maintenance obligation $\Obl^{m}\langle \oblr, \oblt, \obld\rangle$ can be parametrised into $\overline{A}\Delta(\oblr, \oblt, \obld)$  to generate $\Delta$-constraints. With this parametrisation the patterns would be satisfied by the existence of a trace  where $\oblr$ holds when a transition having satisfiying $\oblt$ is executed, and the satisfaction of $\oblr$ is not retracted before the execution of a transition leading to the satisfaction of $\obld$. Such a trace, if it exists, satisfies the given local maintenance obligation.
\end{definition}

To avoid confusion, we refer to the alternative parametrisations for achievement and maintenance obligations as $\widehat{A}\Delta(\oblr, \oblt, \obld)$ and $\widehat{M}\Delta(\oblr, \oblt, \obld)$ respectively. The $\Delta$-constraints from the two adapted parametrisations can be verified using the pattern approach as outlined in Section \ref{sec:patterns_intro}. With the adapted parametrisation, satisfying the new constraints represents that there exists a trace in the WF-Net satisfying the in force instance of the local obligation for the specific \emph{trigger transition} being considered during the evaluation. Thus, when the analysis for a \emph{trigger transition} cannot satisfy any of the patterns, we can label the \emph{trigger transition} as \emph{not executable}, as not being able to satisfy any pattern means that there is no trace in the model satisfying the in force instance of the local obligation that includes this trigger transition.

After executing the patterns approach, and assigning the \emph{not executable} labels, we can determine whether the WF-Net is partially compliant as follows:

\begin{itemize}
\item Apply an \emph{erase} procedure\footnote{Let \emph{erase} be a procedure that when applied to a process block, it removes the block from the process and is recursively applied to its parent process block. This procedure stops without removing the process block when applied to a type \kwd{XOR}.} to the transitions labelled \emph{not executable}. The effect of this procedure is removing executions from the model containing these \emph{not executable} transitions.
\item If the process block associated to the model is not removed by the \emph{erase} procedure, then there exists a trace of the WF-Net executing only trigger transitions whose in force intervals are satisfiable. For Theorem \ref{the:independence}, this is a sufficient condition to determine that the WF-Net contains a trace satisfying the obligation, hence the WF-Net can be said to be \emph{partially compliant}.
\end{itemize}

%check whether the process allows a trace non containing transitions labelled \emph{not executable}. Such a trace would not trigger in force instances of the local obligation that cannot be satisfied, hence leading to violations. If such a trace exists, then the WF-Net can be declared to be 

%Finally, when a trace in the WF-Net does not contain transitions labelled \emph{not executable}, such model can be considered partially compliant due to Theorem~\ref{the:indep}, stating that if different in force instances of a single obligation are satisfiable, then there exists a trace in the WF-Net satisfying each of these in force instances.

%After adapting the $\Delta$-constraints, the pattern approach can be executed over the tree-like representation of the WF-Net. Using the approach we can label the transitions containing the trigger for the obligation as non executable if the patterns identified by the $\Delta$-constraints are not satisfied. This implies that for the process to be partially compliant there must exist an execution avoiding such labelled transitions.

%Finally, if after executing the patterns approach and assigning the non executable labels the process still allow a valid execution, then the WF-Net can be said to be partially compliant following Theorem~\ref{the:indep}, stating that in force intervals allowing to be satisfied by some executions of the model, do not interfere with the satisfaction of other in force intervals of the same obligation.



\begin{theorem}[Instance Independence]\label{the:independence}
Given a WF-Net $\petri$, and an obligation $\Obl^o(\oblr, \oblt, \obld)$, let $\mathbb{T}$ be the set of transitions in $\petri$ containing $\oblt$ in their annotation. If for each transition in $\mathbb{T}$, there exists a trace in $\petri$ satisfying the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ originating from that transition, then there exists a trace in $\petri$ compliant with  $\Obl^o = \Obl(\oblr, \oblt, \obld)$.
\end{theorem}

Before proceeding with proving the correctness of Theorem \ref{the:independence}, we first introduce the notion of \emph{restricted compliance}.

\begin{definition}[Restricted Compliance]\label{def:restricted}
Given a WF-Net $\petri$, and an obligation $\Obl^{o}\langle \oblr,$ $\oblt,$ $\obld\rangle$, let $\mathbb{T}_\oblt$ be the subset of transition in $\petri$ such that $\forall t \in \mathbb{T}_\oblt$, the annotation of  $t$ satisfies $\oblt$.

We say that a trace $\trace$ of $\petri$ is \emph{restricted compliant} with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T}_r$, written $\trace \models_{\mathbb{T}_r} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$, where $\mathbb{T}_r \subseteq \mathbb{T}_\oblt$, if and only if $\forall t$ such that $t \in \trace$ and $t \in \mathbb{T}_r$, $\trace$ satisfies the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ originating from $t$


%, let $\mathbb{T} : t_1, \dots, t_n$ be a set of transitions in $\petri$ such that each of those transitions contain the trigger $\oblt$ of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ in its annotation. A trace $\trace$ of $\petri$ is restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T}$ (denoted $\trace \models_{\mathbb{T}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$), iff $\forall t_i \in \mathbb{T} \cap \trace,$ $\trace$ satisfies the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ originating from $t_i$.

% $$\forall t_i \in \mathbb{T} \cap \trace, \trace \mbox{ satisfies the in force instance of } O \mbox{ originating from } t_i$$

% and is written as:

% $$\trace \models_{\mathbb{T}} O$$

\end{definition}

Restricted compliance becomes equivalent to check compliance of a trace (Definition~\ref{def:obligations}) when $\mathbb{T}_r \equiv \mathbb{T}_\oblt$. Otherwise restricted compliance only requires that the in force intervals originating from transitions included in the restricted set $\mathbb{T}_r$ are satisfied. From Definition~\ref{def:restricted} we can derive the trivial case where $\mathbb{T}_r = \emptyset$, and every trace would always be restricted compliant with respect to the empty set. Generalising, we can say that a trace is always restricted compliant with a restricted set $\mathbb{T}_r$ if none of its transitions are in $\mathbb{T}_r$. We use the concept of restricted compliance in the proof of Theorem~\ref{the:independence}, Corollary~\ref{the:transitive_independence}, and Lemma~\ref{the:pair_independence}.

%From Definition \ref{def:restricted}, a trace \emph{restricted compliant} with respect to a transition not included in the trace is considered to comply with it, which follows directly from Definition \ref{def:obligations}. Note that the borderline case where a trace does not contain any of the transitions specified in the set, is considered to be restricted compliant with them. We use the concept of restricted compliance in the proof of Theorem \ref{the:independence}, Corollary \ref{the:transitive_independence}, and Lemma \ref{the:pair_independence} .

%The borderline case, where an execution can be restricted compliant with respect to a set of transitions by not containing any of them. Restricted compliance is extensively used by the Corollary \ref{the:transitive_independence}, and Lemma \ref{the:pair_independence} used to prove the correctness of Theorem \ref{the:independence}.

\begin{proof}
We prove the correctness of Theorem \ref{the:independence} by induction:

% \begin{description}
% \item[Base Case ($n=2$)]: 
\vspace{6pt}
\noindent {\bf Base Case ($n=2$)}: given two transitions $t_1, t_2$ in a WF-Net $\petri$ satisfying the trigger of the obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, there exists a trace $\trace$ of $\petri$ such that $\trace \models_{\{t_1, t_2\}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.
%
%for each $t_1, t_2$, that transition is either in the execution and the originating in force interval of $O$ is satisfied, or the transition is not contained in the execution.
%
The correctness of the base case follows directly from Lemma \ref{the:pair_independence}.
\vspace{6pt}

% \item[Induction Step ($n>2$)]: 
\noindent {\bf Induction Step ($n>2$)}: given a set of transitions $t_1, \dots, t_n$ in a WF-Net $\petri$ satisfying the trigger of the obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, there exists a trace $\trace$ of $\petri$ such that $\trace \models_{\{t_1, \dots, t_n\}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$. 
%for each $t_1, \dots, t_n$, that transition is either in the execution and the originating in force interval of $O$ is satisfied, or the transition is not contained in the execution.
%
%Assuming that for $n=k$ there exists an execution containing some of the transitions in $t_1, \dots, t_k$ and satisfying the in force instances of $O$ originating from them, and avoiding the other transitions.
%
Considering now the case $n+1$ where the transition $t_{n+1}$ is considered, Corollary \ref{the:transitive_independence} ensures the existence of a trace $\trace'$ of $\petri$ such that $\trace' \models_{\{t_1, \dots, t_n, t_{n+1}\}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.
%satisfying every in force instance for a set of transitions $t_1, \dots, t_{k+1}$, either by executing them and satisfying their related in force instance of $O$, or avoiding them.

%%%

% \end{description}
\vspace{6pt}

Since both the base case and the inductive step have been proved as true, by mathematical induction, Theorem \ref{the:independence} is then correct.% be generalised to any number of transitions in a model satisfying and rising in force instances of an obligation.%, related to the transitions in the WF-Net 
\end{proof}


\begin{lemma}[Pair Independence]\label{the:pair_independence}
Given a WF-Net $P$ and an obligation $\Obl^o = \langle \oblr, \oblt, \obld\rangle$, for every pair of transitions $t_1, t_2$ in $\petri$, where the annotations of $t_1, t_2$ satisfy the trigger $\oblt$ of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, if there exists a trace in $\petri$ satisfying the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ activated in $t_1$, and there exists a trace in $\petri$ satisfying the in force instance activated in $t_2$, then there exists a trace $\trace$ in $\petri$ such that $\trace \models_{\{t_1, t_2\}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.
%satisfying the in force instance of $O$ activated in $t_2$, then there exists a trace in $P$ having either of the following properties:

%\begin{enumerate}
%\item such trace contains both $t_1$ and $t_2$, and satisfies both instances.
%\item such trace contains either $t_1$ or $t_2$, and satisfies the related activated instance.
%\end{enumerate}
\end{lemma}

We prove the correctness of the lemma for each of the two types of obligations: achievement and maintenance.

\begin{proof}
\noindent\textit{Achievement}
\begin{enumerate}
\item From the premise and Definition~\ref{def:obligations}, describing the semantics of an obligation, we have that there are two in force instances of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, one starting in $t_1$ and one starting in $t_2$.
\item If these two instances are overlapping, then from Lemma \ref{lem:overlapping} we know that both are satisfied. Therefore, in this proof we only consider the \emph{not overlapping} case.\footnote{Remember that an in force instance for an achievement obligation is considered the interval between the trigger and the state where the obligation is achieved, or between the trigger and the state where the deadline is achieved, failing the obligation.% \red{add discussion earlier on in force part}
}
\item Considering only the literals relevant for obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, we have 4 possible states worth considering: $(\oblr, \obld); (\oblr, \neg \obld); (\neg \oblr, \obld); (\neg \oblr, \neg \obld)$. Notice that we do not need to keep track of the literal $\oblt$, as in this case it is only relevant in the annotation of the transition known to be triggering the second instance of $O$. 
%Note that considering the literal $\oblt$ in the state is irrelevant as from the premise we know that the next one appearing is the one triggering the second instance of $O$.
\item The possible states after the first in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ among the 4 considered in (3) are the ones resulting from satisfying the instance, which are: $(\oblr, \neg \obld)$ when only the required event occurs, and $(\oblr, \obld)$ when both the required event and the deadline occur at the same time.
\begin{itemize}
\item $(\neg \oblr, \obld)$: This cannot be true at the end of the first in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, because the in force instance must be satisfied and $\neg \oblr$ with $\obld$ means that the in force interval terminated at the deadline without finding the required event, meaning that the instance has not been fulfilled.
\item $(\neg \oblr, \neg \obld)$: This state cannot be true at the end of the first instance, as either one of the two events are required to terminate the in force interval in either a satisfying or failing way.
\end{itemize}
\item From the premise we know that the second in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ allows a trace to satisfy it. Given the possible state $(\oblr, \neg \obld)$ resulting from the first instance, identified in (4), the second in force instance would be satisfied. Therefore we consider the possible cases which would always allow the second in force instance to be falsified:
\begin{enumerate}
\item The first case we consider requires to execute a transition having $\neg \oblr$ annotated before the execution of $t_2$. This would allow the second in force instance not to be immediately achieved. Additionally, no transition with $\oblr$ annotated must be executed within the in force instance before its termination.
\begin{itemize}
\item Considering the case where a transition having $\neg \oblr$ annotated is executed before $t_2$, if this would be unavoidable, and no transitions having $\oblr$ annotated can be executed after $t_2$, then the second in force instance would not allow to be satisfied by any trace of the model, contradicting the premise.

The only case allowing a transition having $\neg \oblr$ annotated being unavoidable between the execution of the first in force instance and the second, is that $t_1$ is contained in an $\kwd{XOR}$ block. However this case would allow a trace avoiding $t_1$, therefore avoiding the transition having $\neg \oblr$ annotated. Moreover from the premise we know that one of such traces avoiding $t_1$ must satisfy the second in force instance. 

Finally we can conclude that in this case both instances can be considered satisfied by a single trace, as a trace avoiding to activate an in force instance of an obligation by avoiding its trigger transition, it is considered to be restricted compliant with it.
\end{itemize}
\item The second case we consider requires to execute a transition having $\neg \oblr$ annotated before the execution of $t_2$, and requires the execution of a transition having $\obld$ annotated before the execution of $t_2$. This would allow to violate the second in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ as soon as $t_2$ is executed.
\begin{itemize}
\item If the transitions having respectively $\neg \oblr$ and $\obld$ annotated would be unavoidable after the execution of $t_1$, then in the case when also $t_1$ would be unavoidable in every trace, we could conclude that no trace would satisfy the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ in $t_2$. However this contradicts the premise that such a trace exists.

Therefore, we can assume that $t_1$ is avoidable, meaning that it is in an \kwd{XOR} block. From this it follows that there exists a trace avoiding $t_1$, and therefore avoiding the two transitions having respectively $\neg \oblr$ and $\obld$ annotated that would have been unavoidable if $t_1$ would have been executed. Moreover, from the premise we know that one of such traces avoiding $t_1$ must satisfy the second in force instance. 

Finally, we can conclude that in this case there exists a trace restricted compliant with the two trigger transitions.

% both instances can be considered satisfied by a single trace, as an execution avoiding to activate an in force instance of an obligation is considered to satisfy it.
\end{itemize}
\end{enumerate}
\item From the premise we know that the second in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ allows a trace to satisfy it. Given the possible state $(\oblr, \obld)$ resulting from the first instance, identified in (4), the second in force instance would be satisfied. Therefore, we consider the possible cases which would always allow the second in force instance to be falsified:
\begin{enumerate}
\item The case allowing the second in force instance to not be satisfiable would require to have an unavoidable transition executable between $t_1$ and $t_2$ that have $\neg \oblr$ annotated. However, such case can be reduced to the case discussed in (5).(b), which means that there would be a trace avoiding the first in force instance and satisfying the second. 

Similarly, consider the second possibility where also a transition having $\neg \obld$ must be executed between $t_1$ and $t_2$, and after $t_2$ no executable transitions can achieve $\oblr$. This case can be reduced to the one discussed in (5).(a), which means that there would be a trace avoiding the first in force instance and satisfying the second. As such, for this case there exists a trace restricted compliant with both trigger transitions.%either a satisfying both, or one of the instances can be avoided, leading to an execution technically satisfying both instances.
\end{enumerate}
\item Having shown that every possible scenario falsifying the theorem also falsifies its premises, we can then conclude that the theorem is correct for the case where the obligation is of the achievement type.
\end{enumerate}
\end{proof}

\begin{proof}
\noindent\textit{Maintenance}
\begin{enumerate}
\item From the premise and Definition~\ref{def:obligations}, describing the semantics of an obligation, we have that there are two in force instances of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, one starting in $t_1$ and one starting in $t_2$.
\item If these two instances are overlapping, then from Lemma \ref{lem:overlapping} we know that both are satisfied as they are independently satisfied. Therefore, in this proof we only consider the \emph{not overlapping} case.
\item Considering only the literals relevant for obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, we have 4 possible states worth considering: $(\oblr, \obld); (\oblr, \neg \obld); (\neg \oblr, \obld); (\neg \oblr, \neg \obld)$. Notice that we do not need to keep track of the literal $\oblt$, as in this case it is only relevant in the annotation of the transition known to be triggering the second instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$. 

%that considering the literal $\oblt$ in the state is irrelevant as from the premise we know that the next one appearing is the one triggering the second instance of $O$.
\item The only possible state after the first in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ among the 4 considered in (3) is $(\oblr, \obld)$, as from the premise the instance must be satisfied. 
\begin{itemize}
\item $(\oblr, \neg \obld)$ and $(\neg \oblr, \neg \obld)$: These states cannot be true at the end of the first in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, because $\obld$ is required to terminate the instance.
\item $(\neg \oblr, \obld)$: This cannot be true at the end of the first in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, because the in force instance must be satisfied and $\neg \oblr$ would prevent that according to Definition~\ref{def:obligations}, describing the semantics of the obligation.
\end{itemize}
\item From the premise we know that the second in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ allows a trace to satisfy it. Given the state from (4) the second in force instance would be satisfied. Therefore we consider the possible cases which would always allow the second in force instance to be falsified:
\begin{enumerate}
\item The first case we consider is where a $\neg \oblr$ must always be the case within the second in force instance after $t_2$ and before any $\obld$ is added to the process state concluding the instance. This allows to falsify the instance in each of its traces.
\begin{itemize}
\item This cannot be the case as it would falsify the premise that the model contains at least a trace satisfying the second in force instance of the obligation.
\end{itemize}

\item The second case allowing only traces falsifying the second in force instance is one where a transition having $\neg \oblr$ annotated must be executed before the second in force instance is activated, and no other transition with $\oblr$ annotated can be executed before the activation.
\begin{itemize}
\item If this case would always be required to be executed in the model, then it would go against the premise that the second in force instance allows a trace satisfying it.
\item Therefore this case must be avoidable. A first possible way is having the transition having $\neg \oblr$ annotated being in an \kwd{XOR} block. However this would make such transition avoidable, meaning that there would be a trace satisfying the second in force instance.
\item The second and last possible way is that the transition $t_1$ activating the first in force instance is within an \kwd{XOR} block with the transition having $\neg \oblr$ annotated.

\begin{itemize}
\item This would allow to have the transition with $\neg \oblr$ annotated being unavoidable after the execution of $t_1$ and the activation of the first in force instance.
\item However this structure would allow a trace avoiding both $t_1$ and the transition having $\neg \oblr$ annotated. Such trace be restricted compliant with both trigger transitions.%would satisfy the second in force instance as for the premise, and also the first as an non activate instance is always considered satisfied.
\end{itemize}
\end{itemize}

%\item \red{no other cases possible}
\end{enumerate}
\item Having shown that every possible scenario falsifying the theorem also falsifies its premises, we can then conclude that the theorem is correct for the case where the obligation is of the maintenance type.
\end{enumerate}
\end{proof}

\begin{corollary}[Transitive Independence]\label{the:transitive_independence}
Given a WF-Net $\petri$, and an obligation $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, let $\mathbb{T} : t_1, \dots, t_n$ be a set of transitions in $\petri$ such that each of those transitions contain the trigger $\oblt$ of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ in its annotation.
%
Let $\Theta$ be a non empty set of traces of $\petri$ such that $\forall \trace \in \Theta, \trace \models_{\mathbb{T}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.

Given a transition $t_{n+1}$ containing the trigger $\oblt$ of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ in its annotation, and not already contained in $\mathbb{T}$, if there exists a not empty set $\Theta'$ containing some traces of $P$ such that $\forall \trace' \in \Theta', \trace' \models_{t_{n+1}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$, then there must exist a set $\Theta''$ containing some traces of $P$ such that $\forall \trace'' \in \Theta'', \exe'' \models_{\mathbb{T} \cup t_{n+1}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.
\end{corollary}

\begin{proof}
We prove the correctness of Corollary~\ref{the:transitive_independence} by contradiction. Let us assume that the set $\Theta'$ is not empty and the set $\Theta''$ is empty.
%
We identify the properties that must hold for $\Theta''$ to be empty by analysing the following complementary subsets of $\Theta$:
\begin{enumerate}
\item Let $\Theta^0$ be a subset of $\Theta$ containing the traces of $\petri$ not containing any of the transitions in $\mathbb{T}$.
\begin{enumerate}
\item If $\Theta^0$ is not empty, then for $\Theta''$ to be empty: the transition $t_{n+1}$ must be included in each of the traces in $\Theta^0$ and the in force instance originating from $t_{n+1}$ must not be satisfied. However this would have $\Theta'$ to be empty, which in turn would \emph{contradict} our opening statement that $\Theta''$ is not empty \textbf{(I)}.

%%%

% If this would not be the case, then there would be a trace not containing any transition in $\mathbb{T}$ and also not containing $t_{n+1}$, which would make this trace restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T} \cup t_{n+1}$, which in turn would \emph{contradict} our opening statement that $\Theta''$ is not empty \textbf{(I)}.
%\begin{enumerate}
%\item For the case where some traces of $\petri$ contain exclusively $t_{n+1}$ and none of the other transitions in $\mathbb{T}$, such traces must not satisfy the in force instance of $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$, otherwise $\Theta''$ would not be empty. The case where some traces of $\petri$ contain $t_{n+1}$ and some of the other transitions in $\mathbb{T}$ is analysed in \textbf{2.(a)} of this proof.
%\end{enumerate}
%\item If $\Theta^0$ is empty, then there cannot be a trace avoiding every transition in $\mathbb{T} \cup t_{n+1}$, and as analysed in \textbf{1.(a).i} of this proof, the traces of $\petri$ containing exclusively $t_{n+1}$ must not be restricted compliant with respect to $t_{n+1}$, and traces also containing some of the other transitions in $\mathbb{T}$ is analysed in \textbf{2.(a)} of this proof.
\end{enumerate}

\item Let $\Theta^n$ be a subset of $\Theta$ containing the traces of $\petri$ that contain a non empty subset of the transitions in $\mathbb{T}$ and $\forall \trace \in \Theta^n$, it is still true that $\trace \models_{\mathbb{T}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$.
\begin{enumerate}
\item If $\Theta^n$ is not empty, then $\forall \trace \in \Theta^n$: $\exe$ must include $t_{n+1}$, otherwise such a trace in $\Theta^n$ not including $t_{n+1}$ would be restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T} \cup t_{n+1}$, and each of these traces containing $t_{n+1}$ must also not be restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T} \cup t_{n+1}$ ($\trace \not \models_{\mathbb{T} \cup t_{n+1}} \Obl^{o}\langle \oblr, \oblt, \obld\rangle$). We analyse the requirements for this to be the case below in two distinct cases:%depending on the type of $O$:
\begin{itemize}
\item When $t_{n+1}$ is executed in a trace before every $t \in \mathbb{T}$, for such case to fail, either a transition being executed after the in force instance originating from $t_{n+1}$ leads to violations in the following in force instances, or a transition executing before or during the in force instance originating in $t_{n+1}$ leads to violating it. The first option cannot be the case, as in that scenario the trace would not belong to $\Theta^n$ as it would not be restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T}$. Meaning that the only possible case is the second option \textbf{(II)}.

\item When $t_{n+1}$ is executed in a trace after one or more $t \in \mathbb{T}$, for such case to fail a transition executed before or within the in force instance originating from $t_{n+1}$ must lead to its violation. These cases are: a transition containing the negation of the requirement being executed within the interval, or before it and not retracted in case of a \emph{maintenance} obligation, and a transition containing the negation of the requirement being executed before the instance and the lack of a transition containing the requirement being executed within the instance \textbf{(III)}.
\end{itemize}
\item If $\Theta^n$ is empty, then it means that $\Theta^0$ must not be empty for $\Theta$ to contain a trace restricted compliant with $\Obl^{o}\langle \oblr, \oblt, \obld\rangle$ with respect to $\mathbb{T}$. Hence the same analysis as the one shown in \textbf{1.(a)} in this proof applies here. %\red{recap the analysis result?}
\end{enumerate}
\end{enumerate}

Following from the analysis above, we can see that \textbf{(II)} leads to the cases analysed in Lemma \ref{the:pair_independence}, which concluded that the in force instances originating from the second transition could not be satisfied by the traces of the model, in this case leading to $\Theta'$ to be empty.

Similarly, when considering \textbf{(I)} and \textbf{(III)} together, they also imply that the requirements for $\Theta''$ to be empty, also require $\Theta'$ to be empty, which again contradicts the premises of the theorem.
 
%\red{conclude the proof by showing that the assumptions leads to $\mathbb{E}'$ to be empty}

\end{proof}

\begin{proof}
\red{revised proof C1}

\red{INTUITION: for $\Theta$ to not be empty and $\Theta'$ to not be empty, $\Theta$ must contain a trace containing a subset of $\mathbb{T}$ where each in force interval from the ones contained is satisfied, and must also contain $t_{n+1}$ and the in force interval originating there must be violated (for $\Theta''$ to be empty). Similarly, $\Theta'$ must contain a trace containing $t_{n+1}$ and the in force instance originating there must be satisfied, while it also contains a non empty subset of $\mathbb{T}$ where at least one of the in force instances originating there is violated. Given these condition, $\Theta''$ cannot be empty as there must exist a trace containing a subset of $\mathbb{T} + t_{n+1}$ where all the in force instances are satisfied.}

\red{The intuition of the proof continues by reasoning that for these particular traces to exist, given the common transitions and the different evaluations of the in force intervals, there must exist in the structure of the model some XOR blocks allowing these traces to exist individually. However these XOR blocks cannot prevent the existence of a trace fitting into $\Theta''$.}

\red{List the trivial cases for which $\Theta''$ is not empty, and analyse in details the one or two cases where the XOR make it a bit more complex.}

\begin{enumerate}
\item If $\Theta$ contains a trace that does not contain $t_{n+1}$, then such trace also belongs both to $\Theta'$ and to $\Theta''$ (from Definition~\ref{def:restricted}).
\item If $\Theta'$ contains a trace that does not contain any of the transitions in $\mathbb{T}$, then such trace also belongs both to $\Theta$ and to $\Theta''$ (from Definition~\ref{def:restricted}).
\item A necessary condition for $\Theta''$ to be empty is that every trace contains the transition $t_{n+1}$ and at least a transition from the set $\mathbb{T}$.
\item Let $\mathbb{T}'$ be a non empty subset of $\mathbb{T}$, and let $\trace$ contain the transitions $\mathbb{T}' + t_{n+1}$. In $\trace$, each in force instance originating from the transitions in $\mathbb{T}'$ is satisfied, and the in force instance originating from $t_{n+1}$ is \emph{not} satisfied. This means that $\trace$ is in $\Theta$ and it is not in either $\Theta'$ or $\Theta''$.
\item Let $\mathbb{T}''$ be a non empty subset of $\mathbb{T}$, and let $\trace'$ contain the transitions $\mathbb{T}'' + t_{n+1}$. In $\trace'$, at least one of the in force instances originating from the transitions in $\mathbb{T}'$ is \emph{not} satisfied, and the in force instance originating from $t_{n+1}$ is satisfied. This means that $\trace$ is in $\Theta'$ and it is not in either $\Theta$ or $\Theta''$.
\begin{enumerate}
\item \red{how do we relate $\mathbb{T}'$ and $\mathbb{T}''$?}
\end{enumerate}
\item Lets consider the following cases: (\red{for simplicity we have 1 violated instance in $\trace'$})
\begin{enumerate}
\item asd
\end{enumerate}
\item asdf
\end{enumerate}

%%%

We prove the correctness of Corollary~\ref{the:transitive_independence} by contradiction. Let us assume that the set $\Theta'$ is not empty and the set $\Theta''$ is empty.

\begin{enumerate}
\item Given the non empty set $\Theta$, for $\Theta''$
\end{enumerate}
\end{proof}
